Learning to Immunize Images for Tamper Localization and Self-Recovery

Digital images are vulnerable to nefarious tampering attacks such as content addition or removal that severely alter the original meaning. It is somehow like a person without protection that is open to various kinds of viruses. Image immunization (Imuge) is a technology of protecting the images by introducing trivial perturbation, so that the protected images are immune to the viruses in that the tampered contents can be auto-recovered. This paper presents Imuge+, an enhanced scheme for image immunization. By observing the invertible relationship between image immunization and the corresponding self-recovery, we employ an invertible neural network to jointly learn image immunization and recovery respectively in the forward and backward pass. We also introduce an efficient attack layer that involves both malicious tamper and benign image post-processing, where a novel distillation-based JPEG simulator is proposed for improved JPEG robustness. Our method achieves promising results in real-world tests where experiments show accurate tamper localization as well as high-fidelity content recovery. Additionally, we show superior performance on tamper localization compared to state-of-the-art schemes based on passive forensics.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> method_backup.tex <==
\begin{figure*}[!t]
	\centering
	\includegraphics[width=1.0\textwidth]{figures/framework_PAMI.pdf}
	\caption{\textbf{Sketch of the pipeline of Imuge+.} IINet is employed to embed slight perturbations into the original images for immunization. Hand-crafted digital attacks in the social medias are decomposed into tampering and post-processing and correspondingly simulated by an attacking layer. Afterwards, a forgery detector helps predicting the tampering mask and removing the tamper from the received image. Finally, the inversed procedures of IINet recovers the original image. We additionally introduce two discriminators to improve the quality of the generated images.}
	\label{fig_framework}
\end{figure*}
% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{figures/couple_layer.pdf}
% 	\caption{Illustration of detaching the attack simulation part from the main-stream.}
% 	\label{fig_components}
% \end{figure}

In this section, we elaborate our method for image immunization and self-recovery. Fig.~\ref{fig_framework} illustrates the network design of Imuge+. We first present the problem statement of image immunization and self-recovery. Then, we show the details of the network architecture and the learning objectives.

\subsection{Approach Overview}
\noindent\textbf{Problem Statement. }
Typical malicious image malipulation attack can be generalized by a function $\emph{Mani}(\cdot)$ in Eq.~(\ref{eqn_tamper}). 
\begin{equation}
\label{eqn_tamper}
\mathbf{X}_{\emph{atk}}=\emph{Mani}(\mathbf{X},\mathbf{M})=\emph{IP}\left(\mathbf{X}\cdot(1-\mathbf{M})+\mathbf{R}\cdot\mathbf{M}\right),
\end{equation}
where $\cdot$ denotes pixel-wise multiplication. $\mathbf{X}$ and $\mathbf{X}_{\emph{atk}}$ are respectively the targeted image and its attacked version. $\mathbf{M}$ is the tampering mask, which is generally the region of interest of $\mathbf{X}$. The contents within the mask are replaced with irrelevant contents denoted by $\mathbf{R}$. $\emph{IP}(\cdot)$ summarizes the image post-processing behaviors such as JPEG compression, rescaling, etc. 
Image tamper localization is to determine the tamper mask $\mathbf{M}$ from the received attacked image $\mathbf{X}_{\emph{atk}}$, and image self-recovery is to take an advanced step to reconstruct the destroyed contents, i.e., $\mathbf{X}\cdot\mathbf{M}$. 
We employ two function $f_{M}(\cdot)$, $f_{\emph{rec}}(\cdot)$ respectively for these two tasks.
\begin{equation}
\label{equation_recovery}
\hat{\mathbf{X}}=f_{\emph{rec}}\left(\mathbf{X}_{\emph{atk}}\cdot\left(1-\hat{M}\right)\right),
\end{equation}
\begin{equation}
\label{equation_tamper_mask}
\hat{M}=f_{\emph{M}}(\mathbf{X}_{\emph{atk}}),
\end{equation}
where $\hat{\mathbf{X}}$ and $\hat{\mathbf{M}}$ are respectively the predicted tamper mask and the reconstructed image.
% , and we expect that $\mathbb{E}(\hat{\mathbf{X}})=\mathbf{X}$ and $\mathbb{E}(\hat{\mathbf{M}})=\mathbf{M}$. 
However, since the non-tampered areas of $\mathbf{X}_{\emph{atk}}$ do not contain any information of $\mathbf{X}\cdot\mathbf{M}$. As a result, if $\mathbf{X}$ in Eq.~(\ref{equation_recovery}) is directly the original image $\mathbf{I}$, it leads to a sub-optimal solution that the destroyed contents will be hallucinated using image prior~\cite{ulyanov2018deep} rather than faithfully recovered.

To address the issue, we employ a third function $f_{prt}(\cdot)$ to embed deep representations of an original image into itself, i.e.,
$\mathbf{X}=f_{\emph{prt}}(\mathbf{I})$ in Eq.~(\ref{eqn_tamper}),
% , where $\mathbb{E}(f_{prt}(\mathbf{X}))=\mathbf{I}$.
% To model the above functions, with Eq.~(\ref{eqn_tamper}), Eq.~(\ref{equation_recovery}) as well as $\mathbb{E}(f_{prt}(\mathbf{X}))=\mathbf{I}$ and $\mathbb{E}(f_{prt}(\hat{\mathbf{M}}))=\mathbf{M}$, we have
% % \mathbb{E}\left(f_{\emph{rec}}\left(\mathbf{X}_{\emph{atk}}\cdot\left(1-\hat{M}\right)\right)\right)
% \begin{equation}
% \label{equation_invertible}
% \mathbb{E}\left(f_{\emph{rec}}\left(\emph{IP}\left(f_{\emph{prt}}\left(\mathbf{I}\right)\cdot\left(1-\mathbf{M}\right)\right)\right)\right)=\mathbf{I}.
% \end{equation}
and formulate $\mathbf{X}=f_{\emph{prt}}\left(\mathbf{I}\right)$ and $\hat{\mathbf{I}}=f_{\emph{rec}}(\mathbf{X}_{\emph{atk}}\cdot\left(1-\hat{\mathbf{M}}\right))$ as a pair of invertible functions, where we expect that $\hat{\mathbf{I}}=\mathbf{I}$ and $\hat{\mathbf{M}}=\mathbf{M}$. In other words, by introducing image self-embedding, we wish to recover $\mathbf{I}$ when the tampered area is detected and removed, even if the self-embedded version $\mathbf{X}$ is attacked with randomized attacking method $\emph{IP}(\cdot)$ and tamper mask $\mathbf{M}$.

\noindent\textbf{Network Modeling. }
Accordingly, we design four phases for Imuge+, namely, image immunization, image redistribution, forgery detection and image recovery. 
We use a single INN network called Invertible Immunization Network (IINet) to model $f_{\emph{prt}}(\cdot)$ and $f_{\emph{rec}}(\cdot)$ simultaneously. Image tampering and post-processing are implemented by an attacking simulation layer which consists of several differentiable methods. A forgery detector is trained for $f_{\emph{M}}(\cdot)$.
We also introduce two discriminators denoted as $\mathcal{D}_A$ and $\mathcal{D}_B$ to respectively distinguish $\mathbf{X}$ and $\hat{\mathbf{I}}$ from $\mathbf{I}$. 
Fig.~\ref{fig_framework} shows a sketch of the pipeline of our scheme. 

Specifically, we transform the original image into the immunized image using the forward pass of IINet. The protected version is uploaded onto the social cloud for daily applications instead of the unprotected original image. To simulate the image redistribution stage, we first perform tampering that evenly varys from splicing, copy-move or inpainting attack. Then, common image post-processing attacks are performed before data storage. On the recipient's side, the forgery detector produces the predicted tamper mask to see which parts of the image are tampered, and we correspondingly remove the tampered contents. Finally, by inversely running the IINet, we reconstruct the recovered images. 
% Note that a wrongly predicted tamper ask during the early training stage will unbalance the invertible function. So we feed the ground-truth rectified image $\hat{\mathbf{X}_{atk}}\cdot(1-\mathbf{M})$ into IINet for self-recovery instead of $\hat{\mathbf{X}_{atk}}\cdot(1-\hat{\mathbf{M}})$. 
% The inputs and outputs of the networks are:
% \begin{equation}
% \left\{  
%              \begin{array}{lr}  
%   \label{forward}
%   \mathbf{X} = \mathcal{P}(\mathbf{I})\\
%   \mathbf{I}_{\emph{atk}}, \mathbf{M} = \mathcal{A}(\mathbf{I}_{\emph{prt
%   }})\\
%   \hat{\mathbf{M}} = \mathcal{F}(\mathbf{I}_{\emph{atk
%   }})\\
%   \mathbf{I}_{rect} = \mathbf{I}_{\emph{atk
%   }}\cdot(1-\mathbf{M})\\
%   \hat{\mathbf{I}} = \mathcal{P}^{-1}(\mathbf{I}_{rect}))
%             \end{array},
% \right.  
% \end{equation}
If the generated images are of high quality, they can evade the classification of the two discriminators.

% It is worth mentioning that in previous INN-based tasks, the input of the forward pass and the output of the backward pass are always identical~\cite{lu2021large} or very close~\cite{xing2021invertible, zhao2021invertible} so that the invertibility can be quickly established. But in Imuge+, the input of the backward pass is the rectified image with contents in the tampered areas nullified, and that is in most cases significantly different from the generated immunized image as the output of the forward pass. Nevertheless, we intend to conceal a representation of the original image into the image itself through $f_{\emph{prt}}(\cdot)$, which is also location-agnostic. As a result, when a part of the immunized image is tampered and the direct information within that area becomes unreliable, we can extract the required information from the rest of the image to restore the destroyed content. Therefore, the invertible function can approximately hold with minimized information loss caused by the image tampering procedures $\emph{Mani}(\cdot)$. 

% We first introduce an U-Net based fine-grained quality assessor $\mathcal{QA}$ to distinguish which parts of the recovered images are indeed "recovered" other than "reconstructed". To do that, the network produces a single-channeled and pixel-wise classification mask which is of the same size of the recovered image. "1" represents "recovered", which forces the main-stream to enhance its performance on image recovery. 
% If a part of $\mathbf{I}_{rec}$ is predicted positive by the $\mathcal{D}$, it suggest the corresponding area is poorly recovered. Therefore, by competing with $\mathcal{D}$, IINet will try better in producing more satisfactory recovered image of higher quality to fool the quality assessor.
% The second adversary is the discriminator $\mathcal{D}$. The job is much simpler compared to $\mathcal{QA}$: it distinguishes whether a given image is an immunized image $\mathbf{I}_{imu}$ or an original image $\mathbf{I}$, and the output of $\mathcal{D}$ is traditional instance-wise binary prediction.

\subsection{Framework Specification}
% In this section, we specify the architecture design of the component networks in Imuge+.
% and presents its advantages over other state-of-the-art methods, especially over Imuge and differentiable JPEG simulators.

\noindent\textbf{Invertible Immunization Network (IINet)}
IINet embeds deep representation of the original image into itself, and conducts self-recovery provided with the rectified image. 
It is empirical that image immunization should not affect normal use of the image.
We accepts the invertible U-shaped network proposed by Zhao et al. \cite{zhao2021invertible}, where the involved wavelet-based blocks can provide empirical biases to decompose the generated features into lower and higher sub-bands. The design helps IINet restrict modifications towards lower sub-bands and conceal the information required by immunization in the higher sub-bands. 
% We apply Spectral Normalization (SN)~\cite{miyato2018spectral} in each block rather than Batch Normalization (BN) in that SN helps stabilizing the training by restricting the Lipschitz constant of the network.

We take the edge map $\mathbf{E}$ of the original image as the additional input into IINet. 
The introduction of the edge map is to aid high-fidelity image recovery, which is inspired by EdgeConnect~\cite{nazeri2019edgeconnect}.
The edge map is a one-channel matrix generated by the canny edge detection algorithm, and therefore the channel number of the input is four. Accordingly, there will be an additional output channel, denoted as $\mathbf{Y}$. We nullify $\mathbf{Y}$ by forcing it to be close to a zero matrix $\mathbf{O}$. In the inversed process, we also feed an extra $\mathbf{O}$ and let IINet output the predicted edge map $\hat{\mathbf{E}}$ along with $\hat{\mathbf{I}}$. 
% The edge map serves as guiding information for IINet to generate a more precise image recovery result.
% Spectral Normalization (SN)~\cite{miyato2018spectral} instead of the traditional batch normalization is adopted in each block, since it helps stabilizing the training.

% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.46\textwidth]{figures/attack_examples.pdf}
% 	\caption{\textbf{Illustration of three kinds of tamper attack simulation (a) splicing, (b) copy-move and (c) inpainting.} The tamper masks are randomly-generated. }
% 	\label{fig_augmentation}
% \end{figure}
% \noindent\textbf{Attack layer} 
\begin{figure*}[!t]
	\centering
	\includegraphics[width=1.0\textwidth]{figures/JPEG_Network.pdf}
	\caption{\textbf{Illustration of the knowledge-distillation-based JPEG simulator (KD-JPEG).} The student/teacher network are respectively provided with the plain-text image and its JPEG version using real-world compressor. The two networks output the generated JPEG images, whose quality factor (QF) are monitored by the QF predictor. The predictor is pre-trained by classifying the real-world JPEG images and guides the generation of the simulated JPEG images. During inference, we only activate the student network.}
	\label{fig_jpeg}
\end{figure*}
\noindent\textbf{Attack simulation.} 
% We simulate several types of image processing attacks as well as malicious tampering according to Eq.~\ref{eqn_tamper}. The attack layer implements five types of attacks and two types of malicious tampers. 
We introduce the malicious attacks before introducing benign post-processing attacks.
To begin with, a number of random areas within $\mathbf{X}$ are selected and tampered according to the tamper mask $\mathbf{M}$. We denote the tampered image before image post-processing attack as $\mathbf{X}_{\emph{tmp}}$, where $\mathbf{X}_{\emph{tmp}}=\mathbf{X}\cdot(1-\mathbf{M})+\mathbf{R}\cdot\mathbf{M}$. The generation of $\mathbf{M}$ is borrowed from DeepFillV2~\cite{yu2018generative}. We restrict the rate of the tampered region as $r_{t}\in[0.0,0.5]$. To simulate copy-move attack, we let $\mathbf{R}$ in Eq.~(\ref{eqn_tamper}) as a spatially-shifted version of $\mathbf{I}_{M}$, which also contains the embedded information. To simulate splicing attack, we simply use another clean image for replacement. To simulate inpainting attacking, we use the open-source model from DeepFillv2~\cite{yu2018generative} to generate the inpainted result as $\mathbf{R}$. The three kinds of tamper are iteratively and evenly performed for a balanced training. 
Note that minimizing the false alarm rate is also important for computer vision tasks. Accordingly, we force Imuge+ to predict a zero matrix for tamper localization when there is no tampering attack, i.e., $r_{t}=0$ and $\mathbf{X}_{\emph{tmp}}=\mathbf{X}$.
% Fig.~\ref{fig_augmentation} shows three examples of tamper simulation for training our Imuge+.
% Note that different from real-world tamper attack, we randomly attack the image by the free-form tamper mask. Therefore, Imuge+ must learn to protect the whole image instead of paying attention to the potential region of interests.

% \noindent\textbf{Image post-processing simulation.} 
After image tampering, we implement the most-commonly-seen image post-processing attacks to simulate that the attacker wants to conceal the tampering behavior. $\mathbf{X}_{\emph{atk}}=\emph{IP}(\mathbf{X}_{\emph{tmp}})$. The image post-processing attacks include Addition of White Gaussian noise (AWGN), Gaussian blurring, image rescaling, lossy image compression represented by using the JPEG standard, Median filtering and cropping. Note that if $\mathbf{X}$ is cropped, the recipient only localizes tamper and recovers the original contents within the cropped area.

Finally, both $\mathbf{X}$ and $\mathbf{X_{\emph{atk}}}$ are required to be converted into 8-bit RGB format. We perform two-round image quantization where we adopt the Straight-Through Estimator~\cite{bengio2013estimating} to calculate the approximate gradients for the rounding operations.
% There are more kinds of attacks such as image hue adjustment, contrast enhancement, brightness change, etc., but we only introduce the above-mentioned six types of attacks as the most representative. 
% Besides, though drop-out attack is not likely to happen in the real world in that the attacker rarely has the original version of the modified image and therefore he cannot revert the pixels, previous works have proven than introducing dropout attack as adversarial training helps boosting the performance. Similar to the drop-out technique used on the model parameters, it forces the network to learn a more robust representation for the tasks and neglect pixel-wise perturbations.

\noindent\textbf{Knowledge-distillation-based JPEG simulator.}
There are already many schemes which include a carefully-designed JPEG simulator, e.g., Diff-JPEG~\cite{shin2017jpeg}, MBRS~\cite{jia2021mbrs} and HiDDeN~\cite{zhu2018hidden}. However, the real-world JPEG robustness of these schemes is still limited. 
It mainly attribute to that neural networks can over-fit fixed compression mode where the above-mentioned works use limited number of quantization tables. In contrast, the quantization table in real-world JPEG images can be customized and flexibly controlled by the quality factor as well as the image content. 
% For example,~\cite{zhu2018hidden,zhu2018hidden} uses a fixed quantization table to mimic JPEG compression while in the real world the quantization table is not fixed.
We present a novel knowledge-distillation-based JPEG simulator using a novel JPEG generative architecture to alleviate this issue.
Fig.~\ref{fig_jpeg} illustrates the network design of the JPEG simulator, which consists of three parts, namely, a real-world JPEG compressor, a QF predictor, and a pair-wise student and teacher network.

First, we use the FFJPEG library to store the plain-text images $\mathbf{I}$ in JPEG format as the ground-truth JPEG-compressed images $\mathbf{I}_{\emph{jpg}}$, with QF arbitrarily assigned. 
% The two networks are respectively provided with $\mathbf{I}_{\emph{jpg}}$ and $\mathbf{I}$, and they individually generate $\mathbf{I}_{\emph{jpg}}$. 
We then train the QF predictor to classify $\mathbf{I}_{\emph{jpg}}$ by their QF. 
Afterwards, we train the pair-wise teacher and student network to produce pseudo-JPEG images.
The student network is provided with the plain-text image $\mathbf{I}$ while the teacher network is given with the corresponding real-world compressed image $\mathbf{I}_{\emph{jpg}}$. 
They are to produce $\hat{\mathbf{I}}_{\emph{jpg}}$ and $\hat{\mathbf{I}}_{\emph{jpg}}^{'}$, which should resemble $\mathbf{I}_{\emph{jpg}}$. Since reconstruction is much easier than simulation, knowledge distillation is done by employing a feature consisting loss to minimize the distance between the hierarchical feature maps generated by the two networks.
To further help the student network grasp the characteristics of JPEG compression, such as the filtered higher-band information and the chess-board artifacts, we additionally employ a classification loss where the generated images from the two networks must be correctly classified by the QF predictor.
% We enhance the performance of JPEG simulation by two constraints. First, we encourage the student network to better mimic the intermediate representations generated by the teacher network. The first constrain is very common for knowledge-distillation tasks. Second, we train a QF predictor on the real-world JPEG images to predict the QF of a given image. After the predictor converges, we encourage both the reconstructed JPEG image and the simulated JPEG image to be classified into a same category as the corresponding real-world JPEG image. The characteristics of JPEG images can be better learnt by KD-JPEG if the classification results are consistent.

% The QF predictor is then trained with $\mathbf{X}_{\emph{jpg}}$ and $QF$ to correctly classify the images according to their QF. Here we empirically set $m=6$ and the labels of these classes are ${P}_{QF}=\{10,30,50,70,90,100\}$. We do not introduce more categories such as ${P}_{QF}=\{20,40,...,80,...\}$ in that classification tasks usually requires that the samples from the different categories should be easily distinguishable. However, when an image is compressed using two close QF ($\delta_{QF}<10$), the discrepancy is not significant enough and the network will be more likely to converge. Therefore, we set $\delta_{QF}=20$ among the neighboring categories and allow the network to give an imprecise prediction when the ground-truth QF lies in between two neighboring categories.

The student/teacher network shares the same fully convolutional network (FCN) architecture with eight convolutional blocks. To enable the flexibility of generating JPEG images with varied quality factors, we respectively employ two individual multi-layer perceptrons (MLP)
to learn the mapping functions that output modulation parameter pairs ${a}, {b}$ that control the standard deviation and mean of the features.
The outputs of the leading three convolutional layers of the student/teacher network are therefore as follows. 
\begin{equation}
\phi_{i+1}=\emph{Conv}({a}_{i}\cdot\phi_{i}+{b}_{i}),
\end{equation}
where $\phi_{i}, {a}_{i}, {b}_{i}$ represent the hierarchical deep representations of the two networks and the trainable mean and standard deviation at layer $i$. $i\in[0,2]$. Accordingly,  $\phi_{0}^{\emph{stu}}=\mathbf{I}$ and $\phi_{0}^{\emph{tea}}=\mathbf{I}_{\emph{jpg}}$.
To implement the QF predictor, we consider that the trace for JPEG image classification lies in the high frequencies, we employ in parallel a vanilla convolution layer, an SRM convolution layer~\cite{srmconv} and a Bayar convolution~\cite{bayar2018constrained} layer to depress the main components of the input image. Thereafter, we use a typical down-sampling fully-convolutional network (FCN) followed by MLP. 

After training KD-JPEG, we only activate the student network and feed it with $\mathbf{X}_{\emph{tmp}}$ for JPEG simulation. Consider that $\mathbf{X}_{\emph{tmp}}$ contains more higher-band details compared to $\mathbf{I}$ because of image immunization, we additionally introduce some Additive White Gaussian Noise (AWGN) on $\mathbf{I}$ and encourage the removal of higher-band details including AWGN during training KD-JPEG.

% \noindent\textbf{Two-round quantization. }


\noindent\textbf{Forgery detector. }
\label{section_fogery_detector}
% ---- Note: move to supplementary
% Ideally, forgery detection should be carried out by a sophisticated off-the-shelf network built upon one of the state-of-the-art image forensics scheme such as MantraNet~\cite{wu2019mantra} or DOA-GAN~\cite{islam2020doa}. However, there are certain drawbacks if we follow this intuition. First, in Section~\ref{section_ablation}, we have analyzed that these methods cannot generalize their detection abilities towards a variety of unseen or hybrid attacks. Second, these networks are usually extra deep which are not feasible to be utilized as a composition of an end-to-end framework, otherwise the training will be easily unstable with vanished or exploded gradients. Third, the distribution of the protected image is different to that of the original image in that some perturbations are introduced for image recovery besides forgery detection. Also, the attacked images are usually post-processed using compression or rescaling to hide the tamper behavior, which severely deteriorate the detection accuracy. Therefore, the well-trained state-of-the-art forgery detection networks will be less effective on the attacked images. 
The forgery detector detects the tampered areas within an attacked image. When the tamper attack simulation is skipped, we force the detector to predict a zero matrix to represent that there is no tamper. We implement it using a four-leveled U-Net~\cite{ronneberger2015u} architecture. 

\noindent\textbf{Discriminators}
We employ the U-Net \yingmodification{proposed by Ronneberger~\cite{ronneberger2015u}} as a U-shaped pixel-wise discriminator~\cite{schonfeld2020u} for $\mathcal{D}_{B}$. The goal is to distinguish which part of $\hat{\mathbf{X}}$ is recovered from tamper removal. A high-quality recovery is expected if \yingmodification{the generated images can cause misclassification of} the discriminator. Besides, we use a Patch-GAN discriminator~\cite{isola2017image} for $\mathcal{D}_{A}$.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/data_augmentation.pdf}
	\caption{\textbf{Example of data augmentation by image pre-tampering.} We prevent IINet by relying on image prior by deliberately tampering some of the original images using splicing. These add-ons will be tampered again and IINet is required to recover them.}
	\label{image_data_augmentation}
\end{figure}
\subsection{Objective Loss Function}
\label{section_loss}
The objective functions include the protection loss $\mathcal{L}_{prt}$, the tamper localization loss $\mathcal{L}_{\emph{loc}}$, the recovery loss $\mathcal{L}_{\emph{rec}}$ and the nullification loss $\mathcal{L}_{\emph{null}}$. There is also the simulation loss $\mathcal{L}_{\emph{jpg}}$ exclusively for KD-JPEG. In the below equations, $\alpha,\beta,\gamma,\theta,\eta$ are the hyper-parameters.

The protection loss $\mathcal{L}_{prt}$ and the recovery loss $\mathcal{L}_{\emph{rec}}$ respectively encourage $\mathbf{X}$ and $\hat{\mathbf{I}}$ to resemble $\mathbf{I}$. The two losses consists of two $\ell_1$ image-level distance term, two adversarial loss term, denoted as $\mathcal{L}_{\emph{adv}}^{\mathbf{D}_{A}}$ and $\mathcal{L}_{\emph{adv}}^{\mathbf{D}_{B}}$ and a $\ell_1$ edge-level distance term. We accept the Least Squared GAN loss (LS-GAN)~\cite{mao2017least} for adversarial training.
\begin{equation}
\mathcal{L}_{prt}=\lVert\mathbf{I}-\mathbf{X}\rVert_{1}+\eta\cdot\mathcal{L}_{\emph{adv}}^{\mathbf{D}_{A}}(\mathbf{X}),
\end{equation}
\begin{equation}
\mathcal{L}_{\emph{rec}}=\lVert\mathbf{I}-\hat{\mathbf{I}}\rVert_{1}+\lVert\mathbf{E}-\hat{\mathbf{E}}\rVert_{1}+\eta\cdot\mathcal{L}_{\emph{adv}}^{\mathbf{D}_{B}}(\hat{\mathbf{I}}).
\end{equation}
% \begin{equation}
% \left\{  
%              \begin{array}{lr}  
%   \label{forward}
%   \mathcal{L}_{prt}=\lvert\mathbf{I}-\mathbf{I}_{imu}\rvert+\mathcal{L}_{\emph{adv}}^{\mathbf{D}_{A}}(\mathbf{I}_{imu})\\
%   \mathcal{L}_{\emph{rec}}=\lvert\mathbf{I}-\mathbf{I}_{rec}\rvert+\mathcal{L}_{\emph{adv}}^{\mathbf{D}_{B}}(\mathbf{I}_{rec})
%             \end{array},
% \right.  
% \end{equation}

The localization loss $\mathcal{L}_{\emph{loc}}$ is to minimize the binary cross entropy (BCE) loss between $\hat{\mathbf{M}}$ and $\mathbf{M}$. 
\begin{equation}
\mathcal{L}_{\emph{loc}}=-[\mathbf{M}\log{\hat{\mathbf{M}}}+(1-{\mathbf{M}})\log{(1-\hat{\mathbf{M}}})].
\end{equation}

The nullification loss $\mathcal{L}_{\emph{null}}$
is to nullify the additional output channel of IINet, namely,
\begin{equation}
\label{eqn_student}
\mathcal{L}_{\emph{null}}=\lVert\mathbf{Y}-\mathbf{O}\rVert_{1}. 
\end{equation}

The total loss for Imuge+ is as follows.
\begin{equation}
\mathcal{L}=\mathcal{L}_{prt}+\alpha\cdot\mathcal{L}_{\emph{rec}}+\beta\cdot\mathcal{L}_{\emph{loc}}+\gamma\cdot\mathcal{L}_{\emph{null}}.
\end{equation}
% The settings of $\alpha$, $\beta$ and $\gamma$ are clarified in the experiments.

KD-JPEG is trained ahead of the whole pipeline. First, we use the Cross-Entropy (CE) loss to train the JPEG predictor by classifying the real-world JPEG images. Then, we employ the CE loss, the $\ell_1$ loss as well as the distillation loss to train the student/teacher networks. The total loss for the student network is
\begin{equation}
\label{eqn_jpeg}
\mathcal{L}_{\emph{jpg}}=\lVert\mathbf{I}_{\emph{jpg}}-\hat{\mathbf{I}}_{\emph{jpg}}\rVert_{1}+\epsilon\cdot~\emph{CE}(\hat{\mathbf{Q}}_{s},\mathbf{Q}_{r})+\sum_{i\in [1,3]}\lVert{\phi}_{i}^{\emph{stu}}-{\phi}_{i}^{\emph{tea}}\rVert_{1},
\end{equation}

% When we decompose the tasks according to Section \ref{sec_details}, we let $\beta=0$, and $\mathcal{L}_{\emph{loc}}$ is only back-propagated into $\mathcal{F}$. Also note that $\mathcal{J}$ has fixed parameters and is not trained end-to-end with the main stream.

\begin{figure*}[!t]
	\centering
	\includegraphics[width=1.0\textwidth]{figures/dataset_images.pdf}
	\caption{\textbf{Examples of the tamper dataset.} The images are generated by volunteers using Adobe Photoshop or Microsoft Drawing. Malicious attacks include copy-move, inpainting and splicing. Benign attacks include typical image processings such as JPEG compression, rescaling, etc.}
	\label{img_tamper_dataset_example}
\end{figure*}
\begin{table*}[!t]
    \renewcommand{\arraystretch}{1.3}
	\caption{\textbf{Composition of real-world tamper dataset divided by the tamper rate.} In most cases, people do not modify the images for too much, and the tamper rate is generally less than 0.3, which is consistent with that of many off-the-shelf tamper datasets.}
	\label{table_dataset_distribution}
	\begin{center}
	\begin{tabular}{c|cccc|cccc|cccc}
	\hline
		\multirow{2}{*}{Attack} & \multicolumn{4}{c|}{MS-COCO} & \multicolumn{4}{c|}{ILSVRC} & \multicolumn{4}{c}{CelebA}\\
		& (0,0.1) & (0.1,0.2) & (0.2,0.3) & \textgreater0.3 & (0,0.1) & (0.1,0.2) & (0.2,0.3) & \textgreater0.3 & (0,0.1) & (0.1,0.2) & (0.2,0.3) & \textgreater0.3\\
		\hline
		Copy-move & 203 & 145 & 104 & 64 & 147 & 85 & 54 & 22 & - & - & - & -\\
        % \hline
		Splicing & 168 & 123 & 84 & 66 & 186 & 102 & 75 & 50 & 115 & 73 & 52 & 20\\
% 		\hline
		Inpainting & 270 & 147 & 87 & 63 & 152 & 74 & 67 & 33 & 102 & 63 & 56 & 39 \\
		\hline
	\end{tabular}
	\end{center}
\end{table*}
\subsection{Training Details}
In all networks, we accept the Spectral Normalization (SN)~\cite{miyato2018spectral} instead of Batch Normalization (BN)~\cite{ioffe2015batch} within each block in that SN helps stabilizing the training by restricting the Lipschitz constant of the network within one. Besides, all down-sampling and up-sampling operations are replaced with lossless Haar transformations.
In the following, we clarify the essential training details.

% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{figures/fig5_supple.pdf}
% 	\caption{\textbf{Example of image augmentation based on two-round tamper.} We deliberately tamper the original images by randomly adding irrelevant contents. }
% 	\label{fig_augmentation}
% \end{figure}
\noindent\textbf{Data augmentation by image pre-tampering}.
% Fig.~\ref{fig_augmentation} shows an example of two-round tamper-based data augmentation (DA). 
We observe that simply varying the generated mask is not enough for effective image immunization and self-recovery. 
In many cases, the randomly generated masks are not good enough to cover the regions of interests in the images. Naturally, Deep Image Prior (DIP)~\cite{ulyanov2018deep} can be learnt by networks to recover an approximate version of the original contents with semantic correctness. However, Imuge+ needs to faithfully reproduce the original image without hallucinating the results.
Therefore, how to guide the network to correctly recover the image without using image prior is a big issue.
% When the key contents in the image is tampered, the network will find no clue for their recovery, and therefore results in significant performance drop in this scenario. 
% We believe it is also a key issue of why Imuge~\cite{ying2021image} can only approximately recover the missing contents but lose their higher-band details.

We propose a new Data Augmentation (DA) paradigm by modifying some of the original images in the training sets using simulated splicing. Fig.~\ref{image_different_rate} shows two examples of our DA. After image immunization, we exactly tamper the add-ons during tamper simulation, i.e., the mask of the first-round and second-round tamper is the same. In other words, the introduced contents are automatically set as the regions of interests of the images, and since the rest of the image shows no relation with the add-ons, IINet is forced not to use image prior to recover image but to utilize image immunization to hide information for the recovery. We control the rate of two-round data augmentation by ${r}_{\emph{aug}}$, and empirically find that ${r}_{\emph{aug}}=15\%$ provides the best performance. The reason is that DIP can facilitate the efficient encoding of the image representation.

\noindent\textbf{Asymmetric batch size.} 
In the majority of previous deep-network-based watermarking schemes~\cite{zhu2018deep,jia2021mbrs}, the attack layer always arbitrarily and evenly performs one kind of attack on the targeted images. However, we argue that the iterative training strategy might be sub-optimal in that the network upgrades unevenly and therefore is more in favor of the results under trivial attacks. We propose to enlarge the batch size after attack simulation to balance the results among different attacks in each iteration. Suppose that the original batch size is $n$, we perform each of the six attacks on the $n$ images, where we get $6\cdot~n$ attacked images. Then, we concatenate these images where the batch size for the backward pass becomes $6\cdot~n$. The advantage of the design is that the calculated results are averaged under different attack scenarios, and therefore the deviation among different batches is much smaller compared to the previous behaviors where each batch only meets a single type of attack.

% \noindent\textbf{Detached Attack Simulation.} 
% Therefore, the networks are evenly trained under various kinds of attacks. 

% The attacks are always added after the tampers. We also arbitrarily skip the tamper attack or the benign attack. 

% \noindent\textbf{Short-cutting the attack layer.}
% Normally for previous schemes~\cite{jia2021mbrs,zhu2018deep}, the gradients need to travel through the attack layer. However, many well-crafted simulators are sophisticated and contain operations like soft rounding. Besides, our KD-JPEG as well as the inpainting simulator require a lot of additional parameters, therefore burdening the training process. 
% To alleviate the above drawback, we accept the idea of short-cutting the attack layer proposed by Zhang et al.~\cite{zhang2021towards}. To be specific, the difference between the immunized image and the attacked image can be obtained, and we add this residual to the immunized image to produce the attacked image. We feed this image into the following network, and the difference is that during the backward propagation, the gradient flow will not propagate into the attack layer. Therefore, we do not need to consider the differentiability or the complexity of the attacks. 
% We compare the experimental results using this strategy with those with traditional attack layer flow in the ablation studies (Section \ref{figure_ablation}).

\noindent\textbf{Iterative training.}.
We inherit and improve the task decoupling mechanism from~\cite{ying2021image}. A wrongly predicted tamper ask during the early training stage will unbalance the invertible function. 
% So we feed the ground-truth rectified image $\hat{\mathbf{X}_{atk}}\cdot(1-\mathbf{M})$ into IINet for self-recovery instead of $\hat{\mathbf{X}_{atk}}\cdot(1-\hat{\mathbf{M}})$. 
Therefore, we divide the training process into two stages, where in the first stage we individually train the forgery detector and the rest of the networks. After the generation of $\mathbf{X}_{\emph{atk}}$, the forgery detector generates the predicted tamper mask $\hat{\mathbf{M}}$ and only updates itself by minimizing $\mathcal{L}_{cls}$. On the other hand, we provide IINet with the ground-truth rectified image $\hat{\mathbf{X}}^{G}$ where we assume a perfect tamper prediction. We then update IINet by minimizing the overall loss $\mathcal{L}_{\mathcal{G}}$ with $\alpha=0$. When $\mathcal{L}_{cls}$ converges to a low level, we move on to the second stage by canceling the task decoupling, and the whole pipeline is thus trained together, where $\hat{\mathbf{X}}$ is influenced by the performance of the forgery localization. It helps IINet to adjust with imperfect tamper classification results.


